Social-VRNN: One-Shot Multi-modal Trajectory Prediction for Interacting Pedestrians

Prediction of human motions is key for safe navigation of autonomous robots among humans. In cluttered environments, several motion hypotheses may exist for a pedestrian, due to its interactions with the environment and other pedestrians. Previous works for estimating multiple motion hypotheses require a large number of samples which limits their applicability in real-time motion planning. In this paper, we present a variational learning approach for interaction-aware and multi-modal trajectory prediction based on deep generative neural networks. Our approach can achieve faster convergence and requires significantly fewer samples comparing to state-of-the-art methods. Experimental results on real and simulation data show that our model can effectively learn to infer different trajectories. We compare our method with three baseline approaches and present performance results demonstrating that our generative model can achieve higher accuracy for trajectory prediction by producing diverse trajectories.

==> sec/01-Intro.tex <==
% !TEX root = ../main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

%This work expands the navigation formulation presented by \cite{Pfeiffer2017} which has the following drawbacks:
%\begin{enumerate}
%\item Single hypothesis/path prediction which in general ends up optimizing the average behavior rather than learning difficult constraints
%\item Predicted trajectories still result in collision
%\item Environment information and other agent information treated in a different way.
%\item Deterministic predictions. The motion uncertainty is nit modeled.
%\end{enumerate}

%Their current implementation uses but we still need to analyze their influence:
%\begin{enumerate}
%\item Goal information
%\item Other pedestrian information is included such as agent velocity
%\end{enumerate}


%What are we going to do? What we want to achieve?
%\begin{enumerate}
%\item Gaussian trajectories
%\item Multi-hypothesis trajectory
%\item Include ego-agent trajectory plan
%\item Collision-free predicted trajectories
%\item Include semantic info instead of goal information? (Sukrit)
%\end{enumerate}

%Current problems:
%\begin{enumerate}
%\item Should we learn the trajectory distribution on position or velocity space?
%\item Current approach can only learn average values...
%\item Model cannot learn variance propagation over-time effect
%\item Wrong initial batch velocities on the dataset. Maybe start using only real datasets. %According with the literature and my evaluation of performance the use of simulated data and real data only damage the performance of the learned model.
%\end{enumerate}

%Possible novelties for the paper:
%\begin{enumerate}
%\item New attention mechanism to solve the collision problem motivated by the need to use the predicted trajectories for guidance of the robot
%\item Evolve the baseline following the state-of-art approaches for multi-hypothesis prediction and integrate them with a motion planner
%\item Implementation of a real-robot with real data
%\item Adapt the prediction models to a new scenario like vessel trajectory prediction
%\end{enumerate}

\section{Introduction}\label{sec:intro}

%WHat is the problem
%\wei{I will rewrite your intro: One of the key features required in autonomous navigation systems to successfully navigate in crowded environments is the ability to predict the other agent's behavior effectively. The successful introduction of mobile robots in human environments is strongly dependent on their ability to reason about the other agent intentions and to forecast their motions. Such skill will allow state-of-art motion planning algorithms to generate safe and socially compliant motion plans for a vast number of applications ranging from service robots to autonomous driving. }
Prediction of human motions is key for safe navigation of autonomous robots among humans in cluttered environments.
%To predict pedestrians behavior is the key for efficient autonomous navigation in clutter environment.
Therefore, autonomous robots, such as service robots or autonomous cars, shall be capable of reasoning about the intentions of pedestrians to accurately forecast their motions. Such abilities will allow planning algorithms to generate safe and socially compliant motion plans. 
% Especially in the scenario of interaction with human, the autonomous robots should be able to predict human motions in order for safe navigation.


%in such environments even with perfect predictions, the state-of-art motion planners may fail under these circumstances due to the Freezing Robot Problem (FRP) if the interaction between the agents is not taken into account \cite{Trautman2010}. The reason is the lack of cooperation which makes the robot believe that no possible path might exist. 
%Why is it interesting/important? E.g. possible applications
%The successful introduction of mobile robots in human environments is strongly dependent on their ability to reason about the other agent intentions and to forecast their motions. \BF{I'll remove this paragraph if necessary due to space limitations}
%Such skill will allow state-of-art motion planning algorithms to generate safe and socially compliant motion plans for a vast number of applications ranging from service robots to autonomous driving. 

%For instance, humans predict the state of environment several steps ahead and plan their motions accordingly.

%to a set of social acceptable rules.


%However, it is intractable to fully enumerate and program all these rules and scenarios into an algorithm to predict their motions.
%freezing robot problem



%Why is it hard / challenging?
The are to key aspect To build  a model of the pedestrian's motion 
However, building an inference model of human motion is extremely difficult due to its uncertainty and multimodality. The uncertainty is caused by the partial observation of the pedestrians' states and their stochastic dynamics. The multimodality is due to the interaction effects between the pedestrians, the static environment and the non-convexity of the problem. 
For instance, as Fig. \ref{fig:multiple_path_example} shows, a pedestrian can decide to either avoid a static obstacle or engage in a non-verbal joint collision-avoidance maneuver with the other upcoming pedestrian, avoiding on the right or left.
%For instance, as depicted in Fig. \ref{fig:multiple_path_example}, under the same circumstances a pedestrian may follow a different trajectory either to avoid a static obstacle or to engage in a non-verbal joint collision avoidance with the other pedestrian.

%Predicting the future trajectories of agents navigating in an unconstrained crowded environment is challenging due to the different factors influencing their motion and its properties:

%\begin{enumerate}
%    \item \textbf{Interaction}: The motion of each agent influences each other. For instance, humans cooperate to avoid collisions.
%    \item \textbf{Static environment}: The static obstacles surrounding the agent imposes physical constraints on its motion. 
%    \item \textbf{Dynamics}: Each agent has a intrinsic motion model which is kinodynamically constrained.
%    \item \textbf{Stochastic}: Trajectories vary from run to run. For instance the human motion is inherently stochastic. 
%    \item \textbf{Multimodal}: Under the same situation an agent may follow different paths which are also socially compliant.
%\end{enumerate}

%E.g. why do naive approaches fail? Or, what's wrong with previous n solutions?
%\BF{I agree that this paragraph is more RL section but I am following Dariu' s recommend structure that says: E.g. why do naive approaches fail? Or, what's wrong with previous n solutions?}
A large number of high accuracy prediction models have been proposed. However, some of these approaches only predict the mean behavior of the other agents \cite{Pfeiffer2017}. Others apply different techniques to model uncertainty such as ensemble modeling \cite{lotjens2019safe}, dropout during inference \cite{gal2016dropout} or learn a generative model and generate several trajectories by sampling randomly from the latent space \cite{Gupta2018}. Recently, Generative Adversarial Networks (GANs) have achieved state-of-the-art in multi-modal trajectory prediction by randomly sampling the latent space to generate diverse trajectories \cite{amirian2019social}. Yet, these methods have two main drawbacks. First, GANs are difficult to train and may fail to converge during training. Second, they require a high number of samples to achieve good prediction performance which is impracticable for real-time motion planning. Moreover, these approaches assume an independent prior across different timesteps ignoring the existing time dependencies on trajectory prediction problems.

%ensemble modelling is limited to really structured environment, such as driving scenarios, where the different hypothesis can be known a priori.
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{img/multiple_path.pdf}
    \caption{Illustration of a scenario where there are multiple ways that
    two pedestrians can avoid a collision. We present a method
    that given the same observed past, predicts multiple socially
    acceptable trajectories in crowded scenes.}
    \label{fig:multiple_path_example}
\end{figure}

The objective of this work is to develop a prediction model suitable for interaction-aware autonomous navigation.
% In this paper, we aim to develop a prediction model suitable for autonomous navigation.
Hence, we  address  these  limitations with a novel generative model for multi-modal trajectory prediction based on Variational Recurrent Neural Networks (VRNNs) \cite{vrnn}. We treat the multi-modal trajectory prediction problem as modeling the joint probability distribution over sequences. To this end, our model first creates a joint representation of three input channels: the pedestrian dynamics, the static environment and other interacting pedestrians. Then, the VRNN structure learns the complex multi-modal distribution conditional to the previous timesteps. Finally, we use a Gaussian Mixture Model (GMM) as output probability model enabling one-shot multi-modal trajectory predictions.
%encoding the uncertainty and multimodality of the data.
%The state-of-art approaches have at least one of the following drawbacks: (i) rely on hand-crafted functions \cite{Helbing1995} - \cite{Kretzschmar2016}
%(ii) do not not reason about static obstacles such
%as the workspace limits or other static obstacles of the robot
%environment \cite{alahi2016social}.


%The existing approaches are limited by at least one of the following shortcomings: (i) The feature functions, which abstract agent trajectory information to an internal representation, are hand-crafted and therefore can only capture simple interactions. (ii) The approaches are not scalable to dense crowds since they use pairwise interactions between all agents [1]–[3], which leads to a quadratic complexity in number of agents, and therefore real-time computation is only feasible for a small number of agents. (iii Static obstacles are neglected [1], [4], [5] and (iv) knowledge about a set of potential destinations is assumed [1], [3], [5].
Our approach makes three key contributions:
 
\begin{itemize}
    \item A new variational deep generative neural network (VDGNN) design for one-shot multi-modal trajectory prediction;
    \item A training strategy is proposed to learn more diverse trajectories in an interpretable fashion;%An efficient sampling approach is proposed by modelling social and environment context as \emph{prior};
   % A sampling approach to generate trajectories from different modes of the probability space accounting for the social and environment context
    \item One-shot prediction model achieving state-of-the-art performance considering a reduced number of samples on both simulated and real datasets. %Highly discriminated trajectories can be predicted compared to state-of-the-art approaches, as demonstrated on both simulated and real datasets;
    %Experimental results on real and simulation data demonstrating the ability of our method to produce diverse trajectories%A simulated dataset to specifically evaluate the multimodality of predicted distributions 
\end{itemize}

%\wei{use passive voice in the following instead of subjective voice}
%Moreover, we present a comprehensive evaluation and comparison against state-of-the-art approaches, for real and simulated data.
%The remainder of the paper is organized as follows: Section \ref{sec:related_work} provides an overview of the related work. Section \ref{sec:preliminaries} introduces the VRNN model. Section \ref{sec:approach} describes the proposed problem and our approach to solving it. Section \ref{sec:experiments} shows our experimental results and Section \ref{sec:conclusion} presents the conclusions of our work.



%What are the key components of proposed approach? Also include any specific assumptions/limitations (don’t leave that for later, or omit altogether)
%The aim of this work is to develop a data-driven model that allows to predict the trajectories of a set of agents. 
%The trajectory prediction problem can be defined as estimating the future states of all agents providing their previous states and environment information.
 
%Our proposed method

%There are three main sources of information which have influence on the agent behavior.
%\begin{enumerate}
%    \item Agent information
%    \item Scene context
%    \item Social context
%\end{enumerate}

%The first consists of information  about the agent path such as previous velocities and position sequences. The second contains the information about the other agents relative to ego-agent like their distance. The last is the information about the environment of the ego-agent like path constraints, obstacles, etc,.



%existing approaches consider an independent prior over time steps not modeling the existing time dependencies

%naive approaches use a high number of mixture components to build a powerful enough to model any dependencies between the components.

%number of parameters scales at least linearly with the number of chosen mixture components

%The remainder of the paper is organized as it follows: Section \ref{sec:related_work} presents an overview of works related to pedestrian trajectory prediction; Section \ref{sec:approach} describes in detail our proposed approach; Section \ref{sec:experiments} provides the experimental results; Section \ref{sec:conclusion} concludes the paper.

==> sec/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

==> sec/expert_knowledge.tex <==
\subsection{Expert Knowledge}
The human navigation behaviour is inherently multimodal. Under the same situation, humans may follow a different path to avoid collision with other obstacles or agents— for instance, Fig. \ref{fig:multiple_path_example} depicts the paths of two pedestrians, in green and purple, constantly switching position from one side of a corridor to the other with an obstacle in the middle of the path. As it can be observed, over time, the same pedestrian may follow a different path under the same circumstance.
Existing approaches for multimodal path prediction either sample from a latent random variable to generate different trajectories (\cite{Gupta2018}) or use ensemble methods (e.g. bagging or bootstrapping) \cite{lakshminarayanan2017simple}. 
In this work, we propose a supervised approach to train a neural network learning to learn how to predict the different possible paths according to the environment setting. Existing public available datasets only provide one of the many possible trajectories that an agent may follow. To avoid the burden of clustering the different followed paths under the same circumstance from a dataset, we resort to a topological path planner (TPP) as the expert. Typically, a TPP combines some motion planner with some metric to classify the generated paths, e.g. winding angles. homotopy classes, etc. In this work, we resort to a homotopy-based TPP. Homotopy classes characterize how paths avoid obstacles allowing to distinguish or group different paths. More specifically, we employ a homotopy-based TPP using A* as the search algorithm, called Homotopy A* (HA*) as presented in \cite{hernandez2015comparison}.
Given a start, a goal position and a grid map containing static and dynamic obstacles, the HA* planner can compute different paths belonging to different classes. We refer to \cite{hernandez2015comparison} for more details about the motion planner.
However, the paths generated by the HA* planner are discrete and kinodynamically different (not "human-like") from a typical human path. Thus, the expert is only used to provide intermediate goal positions from paths belonging to different homotopy classes. Then, the Social Forces model \cite{Helbing1995} is applied to simulate the dynamics of the pedestrian from its current position to an intermediate position. If the obtained path belongs to a different class from the path in the dataset, then it is added to the dataset. Thereby, the original dataset is enlarged with other human-like paths. A summary of the proposed approach is presented in Algorithm \ref{alg:expert}. The algorithm is provided with a dataset, a maximum number of homotopy classes, $M$, to search and a horizon length $T$. The dataset contains the trajectories for a group of $\textbf{n}$ pedestrians. Then, we iterate over the entire dataset by iterating for each pedestrian $i$ and for each time instant $t$ of the recorded trajectory. The function $ \textbf{NextTraj}$ returns two two results cropped segments of $T$ seconds starting from $t_0$ 
%In \cite{Gupta2018}, Gupta et. all. generate $k$ trajectories per scene by randomly sampling $z$ from $\mathcal{N}(0,1)$ in order to avoid that their method to only produce average predictions in cases where there can be multiple hypothesis. 

 
\begin{algorithm}[t]\label{alg:expert}
\caption{Computing different motion hypothesis}\label{expert}
\begin{algorithmic}
    \STATE Given Dataset, $M$ and $H$
    \FOR{$i = 1,\hdots,\textbf{n}$}
        \FOR{$t = 0,\hdots,N^i$}
            \STATE $[\pazocal{O}_{\textrm{static},t}^i, \boldsymbol{p}_0] \leftarrow \textbf{NextTraj}(i,t)$
            %\STATE Given $\pazocal{O}_{\textrm{static},t}^i, [\boldsymbol{p}_t^i,\dots \boldsymbol{p}_N^i]$
            %\STATE $\boldsymbol{p}_0 \leftarrow [\boldsymbol{p}_t,\dots,\boldsymbol{p}_{t+H}]$
            \STATE $HC_0 \leftarrow HomotopyClass(\boldsymbol{p}_0)$
            \FOR{$m = 1,\hdots,M$}  
                \STATE $Path_m$ $\leftarrow$ \textbf{HA}*($\pazocal{O}_{\textrm{static},t}^i, \boldsymbol{p}_t^i, \boldsymbol{p}_N^i$)
                \IF{ $HomotopyClass(Path_m) \ne HC_0$}
                    \STATE $\boldsymbol{p}_m \leftarrow\textbf{SocialForces}(Path_m)$
                    \STATE Dataset.push($\boldsymbol{p}_m$)
                \ENDIF
            \ENDFOR
        \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}

Please note that the other pedestrians are also added to the static gridmap.

==> sec/extra.tex <==
\subsection{Adversarial Trainning}

Neural networks behave in a interesting way, sometimes classifying with high confidence two similar data samples in a different way. An adversarial example shows this case. Adversarial examples, are examples created from the training data by adding the input gradient, the direction of increasing cost. The resulting example is most likely misclassified and so the network is trained to correct such mistakes\cite{goodfellow2016deep}

\subsection{GAN - Multipath prediciton}
Frequently, the solution for a motion planning task has more than one correct answer. For that purpose, models minimizing the MSE between the ground truth and predicted trajectory that an agent performs in some specific situation cannot learn multiple options that the agent may had followed. Generative Adversarial Networks (GANs) are a subclass of generative models enabling multi-modal predictions \cite{Goodfellow2016}.

\cite{goodfellow2014generative} extend the GSN by removing the need of Markov chains.

introduce the adversarial modeling framework consisting on creating a two-player game (competition mechanism) between two networks models: a generative and an discriminative model. In this game, the first tries to
The second tries to discriminate if the data comes from the model or distribution
The competition drives both networks to achieve better results

A \textit{conditional generative model} $p(x|c)$

\subsubsection{Computing different motion hypothesis}
The human motion is inherently multimodal. Given a workspace with obstacles surrounding a query-agent, its start $s$ and goal position $g_i$ it is possible to calculate different path that the agent may have followed. In order to learn this multimodal behavior, first we must reason how to distinguish between different paths. There are several ways to characterize a path. For instance, winding angles, homotopy classes 
In this work we use homotopy classes to classify and compute different paths.


Such paths can be grouped into different categories. There are different

A homotopy class is the set of all possible trajectories from a start to a goal position  that avoid obstacles in the same way. Two paths are homotopic if one can be deformed into the other without intruding an obstacle.

between them For instance, topological path planners such as  given as a local map $\mathcal{M}_i$. The goal position $g_i$ can be obtained from the recorded dataset

\subsubsection{Trajectory classification}

\subsubsection{Trajectory selection}

Previously, we introduced how to generate a set containing trajectories from different homotopy classes according with the topology of the environment. Yet, some of the generated paths are highly unlikely to be followed by the query-agent.

\begin{enumerate}
    \item Velocity direction
    \item Only looking forward
\end{enumerate}

Gradient clipping for the overflow issues.

Adversarial training

\begin{align}\label{eq:biv}
f(x,y) =& \frac{1}{2 \pi \sigma_x \sigma_y \sqrt[]{1-\rho^2}}\exp(-\frac{z}{1-\rho^2})\\
z =& \frac{(x-\mu_x)^2}{\sigma_x}+\frac{(y-\mu_y)^2}{\sigma_y}+2\rho\frac{(x\mu_x)(y-\mu_y)}{\sigma_x \sigma_y} \nonumber
\end{align} 
where the output of the Social LSTM model is composed by five elements: $u_x$, $u_y$, $\sigma_x$, $\sigma_y$ and $\rho$. That represent the mean and standard deviation values of the position variables $x$ and $y$, together with their correlation factor $\rho$.

Noise scheduling technique to encode the uncertainty propagation \cite{Fragkiadaki2015}.

We already use Back-propagation and dropout \cite{hinton2012improving}.

In addition, $\Pi^i_{k,t}$ is the likelihood that the $i$-th agent may follow the $k$-th trajectory at each time step.

%This results in the following input data $\mathcal{D}=(X^{i}_{t-k:t},X^{-i}_{t-k:t},\pazocal{O}^{\textrm{static}})$ to the model. 
%It is assumed a limited number of hypothesis $K$. we denote 
%a set of input and output tuples, $\mathcal{X}$ and $\mathcal{Y}$ respectively.
%The static environment information consists of information about the static environment and the states of the surrounding agents.
%The input is the current query-agent state, the other agents current states and occupancy grid centered on the query-agent, $\mathcal{X}=\{X^{i}_{t},X^{-i}_{t},\pazocal{O}^{\textrm{static}}\}$. The output is the ground-truth trajectory of the query-agent, $\mathcal{Y}=X^{i}_{t:t+\Delta H}$.
%The static environment is represented by an occupancy grid  centered in the query-agent. 
%In order to encode in the model the inherent multimodal behaviour of the agent motion, we express  $X^{i}_{k,t:t+\Delta H}$ as the $k$-th motion hypothesis and $\Pi^i_k$ as the probability weight of the agent following this hypothesis.

The information about the scene is provided as an occupancy map $O_{Static}$. A Convolutional Neural Network (CNN) is pre-trained using a convolutional auto-encoder \cite{cadena2016multi}. The learned encoder network is then later used in the final architecture to extract the most relevant features of the map which is then fed to a LSTM 

Our baseline model consists of 3 separated channel structure incorporating the ego-agent state, environment information and social context. The outputs of each network are concatenated and fed to a sequence of a LSTM plus Fully Connected (FC) network. A s






\subsubsection{Model Training}
At each training iteration a minibatch $y_{Dataset}$ from the dataset and a minibatch $\hat{y}t$ from the model's prediction is drawn. One gradient step is performed to minimize $J_D$ and another to minimize $J_G$. Some works recommend to run more training steps for one player than to the other. (Something maybe to try)

\subsection{MSVRNN model}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/multimodal_network_2.jpg}
    \caption{Multi-space Variational Network architecture}%
    \label{fig:msvrnn}%
\end{figure*}

Homotopy classes allow categorizing different trajectories into different classes. Here, we introduce a multi-space variational recurrent neural network (MSVRNN) for multi-hypothesis trajectory prediction and classification. The likelihood of an agent following a trajectory from a specific class can be described by an additional discrete latent variable $\textbf{y}$ representing the unobserved class of a specific trajectory. Thus, the MSVRNN model combines both continuous and discrete latent variables. We use an additional network to approximate $p(\textbf{y}|\textbf{z})$ working as discriminative classifier. The architecture of the MSVRNN model is presented in Fig. \ref{fig:msvrnn}. 

\subsubsection{Generative Model}
The combined generative model is described as it follows:

\begin{eqnarray}
    %p(\textbf{x}|\textbf{z}_c)=\mathcal{N}(\varphi_{enc}(h_{t-1})) \\
    p_\theta(\textbf{x}_{t+1:t+T}|\mathbf{z}_{c,t})\sim \sum_{m=1}^M\sum_{t=t_0}^{t_0:t_0+T}\mathcal{N}(\mathbf{\mu}_{z,t},\sigma_{z,t}) \\
    p_\pi(\textbf{y}_t|\textbf{z}_{d,t}) = \prod_m^M\textbf{Cat}(y_m|\varphi_{disc}(h_{t-1}))\\ 
    p_{\theta,\pi,\phi}(\textbf{x}|\textbf{y},\textbf{z}) = p(\textbf{x}|\textbf{z})p(\textbf{y}|\textbf{z}) \\
\end{eqnarray}

where $\textbf{Cat}(\cdot)$ is a multinomial distribution encompassing the likelihood of an agent following a specific trajectory over a set of a possible class of trajectories, with $y_m∈\{1,\dots,M\}$. Furthermore, the continuous latent variable is now assumed to be a bivariate Gaussian per time-step over the prediction horizon. Similar to the vRNN model, the convex combination of both models result in a GMM. 

\subsubsection{Prior}

The inference model is the same as defined in Eq. \ref{eq:inf_model}. The key difference between the MSVRNN with the vRNN is the addition of a separated LSTM layer to reason about the trajectory class $y_m$ as depicted in Fig. \ref{fig:network_architecture}. The latent variable is split into a discrete and a continuous $\textbf{z}=[\textbf{z}_d,\textbf{z}_c]$. Thereby, two different priors are assumed over the latent space. 

\begin{eqnarray}
    \textbf{z}_{c,t}\sim \mathcal{N}(\mathbf{\mu}_{0,t},\sigma_{0,t}) \\
    (\mathbf{\mu}_{0,t},\sigma_{0,t})= \varphi_{c,prior}(h^{enc}_t) \\
    \textbf{z}_{d,t}\sim \textit{Gumbel}(0,I)
\end{eqnarray}

To ensure differentiability over the network we employ the Gumbel-Max trick \cite{Tarlow}. Lastly, the outputs of each channel are combined resulting in GMM model. 

\subsubsection{Loss function}
Note that the introduction of discrete latent variables results in a more complex loss function:
\begin{equation}
    \begin{aligned}
        L(\textbf{x},\theta,\phi,\pi) = &\mathbb{E}_{\textbf{z}\sim q_{\varphi_{enc}}(\textbf{z}|\textbf{x})}[\log p_\theta(\textbf{x}|\textbf{z}_c)+\log p_\pi(\textbf{z}_d)] \\ & -\textbf{KL}(q_{\varphi_{enc}}(\textbf{z}_c|\textbf{x})||p(\textbf{z}_c)) \\& 
    \end{aligned}
\end{equation}

 %In order to generate robust predictions the model must reason about the uncertainty associated with the motion of the agent. Thus, to effectively predict the uncertainty we propose a twofold approach. First, similarly to \cite{alahi2016social}, we adapt the output of our baseline network to model the probability distribution of the predicted velocities.
 
\subsection{SRNN - To be completed...}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{img/multimodal_network_srnn.jpg}
    \caption{Network architecture}%
    \label{fig:srnn}%
\end{figure*}

SRNN's combine a deterministic RNN with a State Space Model (SSM) being state-of-art in modelling stochastic sequential processes \cite{NIPS2016_6039}. Our SRNN model follows a similar approach as presented in Fig.\ref{fig:srnn}. We split our network architecture into two main modules: a deterministic and a stochastic. The first is composed by the feature extractor, responsible for pre-processing the input channels as described in section \ref{sec:inputs}, and a deterministic RNN. As previously explained, the deterministic RNN comprising three split LSTM layers followed by a $\textbf{concat}$ operation creates a latent tensor $\textbf{z}$ fusing and encoding the time patterns from the training data.  
The second module, encompassing the stochastic RNN is a SRNN\dots


%In contrast, we model probability density function of next agent velocity conditioned 

%conditioned on the previous agent velocities, social and scene information/context.  in order expand this framework to use the NN to learn the trajectory distribution conditional on the history of previous information.
%As proposed in \cite{bishop1994mixture} the outputs of a neural network (NN) can be used to parameterise a mixture distribution. We follow a similar approach as in \cite{graves2013generating}, which stacks to a a fully-connected layer on the output of a RNN to learn the output distribution. Consider $z$ as the output of our NN baseline

%\begin{equation}
%    P(\hat{v}_{x,t+k},\hat{v}_{y,t+k}|v_{x,t-k:t},v_{y,t-k:t}) \sim \mathcal{N}(\mu^i_{x,k},\sigma^i_k, \rho^i_{y,k})
%\end{equation}

%for $k\in[1,N]$. These parameters are predicted by a Fully Connected (FC) network with an output size $5\times N$. 
 


%Because of the RNN architecture the output distribution is not only conditioned to the actual velocity input, but on the history of previous velocities. The loss function is the negative logarithmic sequence loss:

%\begin{equation}
%    \mathcal{L}=\sum^N_{k=1}-\log\mathcal{N}((v_{t+k}|\mu^i_{x,k},\sigma^i_k, \rho^i_{y,k})
%\end{equation}





%In order to avoid underflow issues due to residual values of the variance or conditional probability training values we apply the \textit{log-sum-trick} \cite{Mooney2012}

%\begin{equation}
%    \mathcal{L}(y|x)=-\log(\sum^N_{k=1}-\log(2\pi \sigma_x \sigma_y\sqrt{1-\rho^2})-\frac{z}{2\sqrt{1-\rho^2}})
%\end{equation}

%Throughout this paper consider $\mu^v_k=(\mu_{v_x,k},\mu_{v_y,k})$ as the expected velocity vector, $\mu^x_k=(\mu_{x,k},\mu_{y,k})$ as the expected position vector and, $\Sigma^v_k$ and $\Sigma^x_k$ as the velocity and position covariance matrix respectively.

%The vRNN-GMM model considers only continuous latent variables. The goal is to find $p(\textbf{x}|\textbf{z},θ) = f(\textbf{x},\textbf{z},\theta)$

%the concatenation of the outputs of each LSTM network $\textbf{z}=[z_i, z_{Static},z_{-i}]$ denoting the latent representation of the agent velocity, static environment and other agent's, respectively:

% \begin{equation}
%     \textbf{z}=
%     \left[
%     \begin{align}
%         LSTM(v_i)\\
%         LSTM(\Phi_{Encoder}(O^{Static}))\\
%         LSTM(\Phi_{O^{-i}}(z_{-i}))
%     \end{align}
%     \right]
% \end{equation}

%with $\Phi_{Encoder}$ and $\Phi_{O^{-i}}$ representing the pre-trained encoder and fully-connected embedding layer functions, respectively.

%As previously stated, we present two possible configurations for the latent space representation resulting in two slightly different network models: a variational recurrent neural network model (vRNN) and a multi-space variational recurrent neural network (MSVRNN).
%In the vRNN-GMM model we consider the feature space to be composed only with continuous latent variables. It introduces a set of vector of latent random variables \textbf{z} capturing the variations in the input variables \textbf{x} and modeling the joint distribution $p(\textbf{x},\textbf{z})=p(\textbf{x}|\textbf{z})p(\textbf{z})$. In vRNN's, the prior on latent random variables, p(\textbf{z}), depend on the previous hidden-state $h_{t-1}$ of the network. The

%while discriminative models (DM's) can learn the likelihood of an agent following a certain trajectory. We leverage this insight when designing our network architecture for multimodal trajectory prediction.

%Social LSTM-based methods output a Bivariate Gaussian distribution \cite{alahi2016social} \cite{Gupta2018} representing the future position for a query-agent over a prediction horizon.

%Our method includes two extensions of previously presented baseline network \cite{Pfeiffer2017}: uncertainty modelling and multi-hypothesis prediction.

%Here, we propose two different network architectures to investigate further the ability of the proposed networks to effectively learn different modal trajectories and its likelihood: one building on variational RNN's and two employing an SRNN as a decoder network.
 
 %We propose two variants for the first architecture, presented in Figure \ref{fig:network_architecture}.  The first uses a single SGM combined with a Gaussian Mixture Model (GMM) as output network. The second, combines an SGM with a stochastic discriminative model, modelling a GMM with two distinct networks, similar to a multi-space variational autoencoders (MSVAEs) \cite{zhou2017multi}.

%%At time $t$, the network derives a hidden state tensor $z_t$ from the input $x_t$. Then, the hidden state is translated to predictions thorough the network output channels, the decoder $\varphi_{dec}$, as follows:

%\begin{equation}
%    \hat{x}_{t+i}=\varphi_{dec}(\textbf{z}_t;\theta_{dec}) \text{for} i \in [1:H]
%\end{equation}
 
%The human motion in constrained environments is influenced by three main factors: the interaction with the other navigating agents, the interaction with the static environment and the agent dynamics
%Considering the surrounding environment in which an agent is moving, there are 
%\subsection{Network Architecture}

%\subsubsection{Features}


%\subsubsection{Time dependecies}
%The problem of forecasting a pedestrian trajectory can be formulated as a sequence modeling tasks. We employ a RNN model to learn the time dependencies . More specifically, we use LSTM neural networks proposed to overcome the issues of RNN with vanishing and exploding gradient problem \cite{goodfellow2016deep}.

%\subsection{Network model}
%In this work, we follow a multi-step prediction strategy by using only current information and the network hidden state to predict more than one time-step. %Thus, the goal is to learn the probability distribution of a sequence with length $H$:

%\begin{equation}
%    p(\textbf{x}_{t:t+H}|\textbf{x}_{t-1})=\prod^H_{k=1}p(\textbf{x}_{t+k}|\textbf{z}_{t+k-1},\textbf{x}_{t})    
%\end{equation}

==> sec/preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminaries}

%\subsection{Nomenclature}

\subsection{Multimodal Trajectory Prediction Problem}\label{sec:problem}

%This paper presents a data-driven approach to predict the uncertain and multimodal pedestrian navigation behavior.
Consider a navigation scenario with $\textbf{n}$ interacting agents navigating on a plane $\pazocal{W} = \mathbb{R}^2$. The dataset $\mathbf{D}$ contains information about the $i$-th agent trajectory $X^i_{1:N}=\{(p_1^i,v_1^i),\dots,(p_N^i,v_N^i)\}$ with $N$ utterances and their surrounding static environment $\pazocal{O}_{\textrm{static}}^i \subset \pazocal{W}$, for $i \in [0, \dots \textbf{n}]$.  Let $\textbf{x}^i_t = \{p^i_t,v^i_t \}$ denote the state of the $i$-th query-agent at time $t$, consisting of the agent position $p^i_t = \{x^i_t,y^i_t \}$ and velocity $v^i_t = \{v^i_{x,t},v^i_{y,t} \}$ with respect to the world frame $\pazocal{W}$. $X^{i}_{t+1:t+T}=(p_{t},\dots,p_{t+T})$ represents the future agent trajectory over a prediction horizon $T$. Throughout this paper the subscript $i$ will denote the query-agent $i$ and $-i$ the collection of all the other agents states. Moreover,  

To account for the uncertainty and multimodality of agent motion, we seek a probabilistic model $f(\theta)$ with parameters $\theta$ over a set of $M$ different trajectories and a prediction horizon $T$:

%The goal is to find a data-driven model with parameters $\theta$ to estimate the conditional probability of the next $n$ agent states: 
\begin{equation}
    \begin{array}{c}
        p(\mathbf{x}^i_{m,t+1:t+T} | \mathbf{x}^{i}_{t},\mathbf{x}^{-i}_{t},\pazocal{O}_{\textrm{static}}) = f(\theta, X^{i}_{t},X^{-i}_{t},\pazocal{O}_{\textrm{static}}) \\

        \forall m \in [0,M]
    \end{array}
\end{equation}
where $m$ is trajectory index and $t$ is query time instant. The probability is conditional to the other agents states and the surrounding environment to models the interaction and environment constraints.
\begin{comment}
    

\subsection{Variational Recurrent Neural Networks}\label{sec:vrnn}
\BF{@Wei Pan: Javier thinks that this is not clear enough and I am not sure weather I should explain it more in detail or just a give a top overview about the method.}
\wei{yes and no. You should start with RNN first. Then say why you want to do variational, because generative blabla, then you say your goal is the generate the time seires/sequence. }
VRNN's are a class of generative models designed to learn the underlying probability distribution of sequential data. The VRNN structure is similar to a VAE composing a generative (encoder) and inference (decoder) model. In contrast to VAE's, the prior over the latent random variable $\mathbf{z}_t$ at time $t$ is conditional dependent on the previous hidden state $h_{t-1}$ of a RNN.  

\begin{equation}
    \begin{split}
        \mathbf{z}_t \sim \mathcal{N}(\mathbf{\mu}_{0,t},\textrm{diag}(\mathbf{\sigma}^2_{0,t})),\\
        [\mathbf{\mu}_{0,t},\mathbf{\sigma}_{0,t}]=\psi^{\textrm{prior}}_\tau(\mathbf{h}_{t-1})
    \end{split}
\end{equation}
with $\psi^{\textrm{prior}}$ is any function approximator such as a neural network, $\mathbf{\mu}_{0,t}$ and $\mathbf{\sigma}^2_{0,t}$ are the mean and variance of the conditional distribution at time $t$ for zero prediction steps, respectively. Moreover, the generation distribution not only depends on the latent random variable $\mathbf{z}_t$ but also on $\mathbf{h}_{t-1}$,being defined as it follows:  

\begin{subequations}
\label{eq-generation}
\begin{align}
    \mathbf{x}_t | \mathbf{z}_t \sim \mathcal{N}(\mathbf{\mu}_{x,t},\textrm{diag}(\mathbf{\sigma}^2_{x,t})) \\
    [\mathbf{\mu}_{x,t},\mathbf{\sigma}_{x,t}]=\psi^{\textrm{dec}}_\tau(\psi^{\mathbf{z}}_\tau(\mathbf{z}_t),\mathbf{h}_{t-1})
\end{align}
\end{subequations}
with $\mathbf{\mu}_{x,t},\mathbf{\sigma}_{x,t}$ as the parameters of the generation distribution, $\psi^{\textrm{dec}}_\tau$ is the decoder model and $\psi^{\mathbf{z}}_\tau$ a feature extractor from the latent space.
The inference model aims to learn the approximate posterior distribution of the latent random variable $\textbf{z}_t$ conditioned on the previous input sequence $\mathbf{x}_{\le T}$:

\begin{subequations}
    \label{eq-posterior}
    \begin{align}
        \mathbf{z}_{\le T}|\mathbf{x}_{\le T} \sim \mathcal{N}(\mathbf{\mu}_{z,t},\textrm{diag}(\mathbf{\sigma}^2_{z,t})) \\
        [\mathbf{\mu}_{z,t},\mathbf{\sigma}_{z,t}]=\psi^{\textrm{enc}}_\tau(\psi^{\mathbf{x}}_\tau(\mathbf{x}_t),\mathbf{h}_{t-1})
    \end{align}
\end{subequations}




\begin{subequations}
    \label{eq-problem}
    \begin{align}
        \mathbf{x}_t | \mathbf{z}_t \sim \mathcal{N}(\mathbf{\mu}_{x,t},\textrm{diag}(\mathbf{\sigma}^2_{x,t})) \\
        [\mathbf{\mu}_{x,t},\mathbf{\sigma}_{x,t}]=\psi^{dec}_\tau(\psi^{\mathbf{z}}_\tau(\mathbf{z_t}),\mathbf{h}_{t-1}) \\
        \mathbf{z}_t | \mathbf{x}_t \sim \mathcal{N}(\mathbf{\mu}_{z,t},\textrm{diag}(\mathbf{\sigma}^2_{z,t})) \\
        [\mathbf{\mu}_{z,t},\mathbf{\sigma}_{z,t}]=\psi^{enc}_\tau(\psi^{\mathbf{x}}_\tau(\mathbf{x_t}),\mathbf{h}_{t-1}) \\
    \end{align}
\end{subequations}


 with $\mathbf{\mu}_{z,t},\mathbf{\sigma}_{z,t}$ are the mean and variance of the approximate posterior distribution, respectively. $\{\psi^{\textrm{dec}}_\tau$ the decoder model and $\psi^{\mathbf{x}}_\tau$ a feature extractor from the input $\mathbf{x}_t$. $\{\psi^{\textrm{dec}}_\tau,\psi^{\textrm{enc}}_\tau,\psi^{\mathbf{x}}_\tau,\psi^{\mathbf{z}}_\tau\}$, can be any function, such as neural networks, allowing to learn complex sequences. Moreover, the VRNN as a RNN updating the hidden-state of the network as it follows:

\begin{equation}\label{eq:vrnn_prior}
    \mathbf{h}_t = f_\theta(\psi^{\mathbf{x}}_\tau(\mathbf{x}_t),\psi^{\mathbf{z}}_\tau(\mathbf{z}_t),\mathbf{h}_{t-1})
\end{equation}

where $f_\theta$ is the transition function of the cell selected for the RNN structure.
\end{comment}
%\subsection{Problem Formulation}

%We assume that the spatial coordinates of all agents and static environment are represented in a local neighborhood of $\textit{E}$, $n_s \times n_s$, centered at the robot's position. %A standard RNN computes a sequence of future pedestrian states $y_t=(x_{t + \Delta t},\dots,x_{t+H})$ for a prediction horizon $H$.
%\begin{align}
%h_t&=sign(W^{hx}x_t+W^{hh}_{t-1})\\
%y+t&=W^{yh}h_t
%\end{align}



%The spatial coordinates of an agent $i$ are expressed in terms of their components $x_t^i$ and $y_t^i$ for each time instant $t$. Besides, a set of positions towards which the robot navigates is also given as the goal information of the robot. Such goal positions are only provided to the ego-agent (robot) and located in parts of the scenario where the robot needs to turn or to encounter an intersection.

%We employ a Recursive Neural Network (RNN) model to observe at each time step $t$ the past positions of all agents from $t-T_{obs}$ till $t$, and estimate the distributions of their positions from $t$ to $t+T_{pred}$. Using for that purpose the goal positions of the robot in that predicted time interval.Therefore, at each time step $t$, the input of our model is composed by the current positions of all agents at current time $t$, the next goal position of the robot, and the memory state of the RNN build from past observations.

%\subsection{Sequence-to-Sequence Model}

%Consider a sequence $\mathcal{P}={P_1,\dots,P_n}$ with $n$ elements and $\mathcal{C^P}={C_1,\dots,C_{m(\mathcal{P})}$ a sequence of $m(\mathcal{P}) \in [1,n]$ indices. A Sequence-to-Sequence neural computes the conditional probability $p(\mathcal{C^P}|\mathcal{P};\theta)$ using a parametric model such as a RNN with parameters $\theta$.

%\begin{equation}
%    p(\mathcal{C^P}|\mathcal{P};\theta)= 
%\end{equation}

%\subsection{Recurrent Mixture Gaussian Network}
%One possible approach is to stack to our network baseline a Mixture Density Network (MDN). A MDN consists



==> sec/problem.tex <==
% !TEX root = ../main.tex

\section{Preliminaries}
\subsection{Mixture Density Network}\label{sec:MDN_pre}

A Mixture Density Network (MDN) is the formulation of a neural network to model the conditional probability distribution of a target dataset $\textit{D}$. The idea behind an MDN is to use the outputs of the network to parameterize a mixture distribution. More specifically, a subset of the outputs is set as the mixture weights and the remaining outputs the respective mixture elements. Consider a neural network with parameters $\theta$ modelling a mixture model conditioned to the input vector $\textbf{x}$ with $M$ components where each component is a Gaussian. 
\begin{equation}
    p(y|\textbf{x},\theta) = \sum_{m=1}^M\pi_m(\textbf{x}) \cdot \mathcal{N}(y;\mu_m(\textbf{x}),\sigma_m^2(\textbf{x})))
\end{equation}

with $\pi_m, \mu_m, \sigma_m$ as the $m$-th mixture weight, mean and variance, respectively. Then, the output vector $\hat{y}=[\hat{\pi}_1, \hat{\mu}_1, \hat{\sigma}_1 \dots \hat{\pi}_m, \hat{\mu}_m, \hat{\sigma}_m]$ is parameterized as it follows:

\begin{subequations}\label{eq:control_problem}
\begin{align*}
\pi_m &= \frac{\exp(\hat{y}_{m})}{\sum_m^M\exp(\hat{y}_{5*l})} \implies \pi_m \in [0,1] \\ 
\mu_m(\textbf{x}) &= \hat{y}_{2*m}  \\
\sigma_m(\textbf{x}) &= \exp(\hat{y}_{3*m}) \implies \sigma_m >0 \\
\end{align*}
\end{subequations}

The goal is to find the set of parameters $\theta$ of the MDN which minimize the negative log-likelihood given the set of input/output pairs in the training dataset $\textit{D}=\{(x_1,y_1),\dots,(x_N,y_N)\}$ with $N$ samples:

\begin{equation}
    \theta^* = \arg \min -\sum^N_t\sum^M_m  \log{p(y_t | x_t,\theta)}
\end{equation}

\subsection{Uncertainty Propagation}
To compute the resulting trajectories we use a linear model with uncertainty resulting in the following dynamical system:

\begin{equation}
    \begin{array}{lc}
        X_{k+1}=x_k+v_k*\delta t & v_k \sim \mathcal{N}(\mu^v_k,\Sigma^v_k)   \\
        \mu^x_{k+1} =\mu^x_k + \mu^v_k*\delta t  &  \\
        \Sigma^x_{k+1} = \Sigma^x_k + \Sigma^v_k *\delta t^2 \\ 
        X_0 \sim \mathcal{N}(\mu_{x,0},\sigma_{x,0}) & \text{Prior  on agent position} \\
        v_0 \sim \mathcal{N}(\mu_{v,0},\sigma_{v,0}) & \text{Prior  on agent velocity}
    \end{array}
\end{equation}

\subsection{Trajectory prediction}\label{sec:rnns}
Recurrent neural networks have demonstrated high efficiency learning time-dependent sequences. When predicting sequences, there are three main approaches which can be followed: many-to-many, one-to-many and recursive. In the first two configurations, the network is requested to predict more than one time-step into the future, differing on the number of past inputs feed to the network. The last learn to predict only a single step using the predicted values to predict the following steps. It has been proven that many-to-many or one-to-many achieve higher prediction performance than recursive approaches. Thus, in this work, we focus ou attention to one-to-many models.
Consider that dataset $D$ from subsection \ref{sec:MDN_pre} is divided into batches of input/output sequences with length $T$.  Given a sequence of inputs $x_{t:t+T}$ at time $t$ a LSTM network predicts a sequence of outputs $\hat{y}_{t+1:t+T}$ by iteratively computing the following equation:

\begin{subequations}\label{eq:lstm}
\begin{align}
    h_t = LSTM(h_{t-1},\theta) \\
    \hat{y}_{t+1:t+T} = \theta_{hy}h_t + b_y
\end{align}
\end{subequations}

where $\theta$ denotes the network weights, $\theta_{hy}$ and $b_{y}$ the weight matrices and the bias vector from the output layer, and $h_t$ the hidden state representing the memory of the network of the past inputs. Three gate mechanisms compose the LSTM function: an input gate $i$, forget gate $f$ and output gate $o$. And, a cell state $c$. Thus, the LSTM equations are described as follows:

\begin{subequations}\label{eq:lstm}
\begin{align}
    i_t = \sigma(\theta_{xi}x_t + \theta_{hi}h_{t-1}+\theta_{ci}c_{t-1}+b_i) \\
    f_t = \sigma(\theta_{xf}x_t + \theta_{hf}h_{t-1}+\theta_{cf}c_{t-1}+b_f) \\
    c_t = f_t c_{t-1}+i_t\tanh{(\theta_{xc}x_t + \theta_{hc}h_{t-1}+b_c)} \\
    o_t = \sigma(\theta_{xo}x_t + \theta_{ho}h_{t-1}+\theta_{co}c_{t-1}+b_o) \\
    h_t = o_t \tanh{c_t}
\end{align}
\end{subequations}
with $\sigma(\cdot)$ as the sigmoid activation function. Typically, the mean square error is defined as the loss function:
\begin{equation}
    L(y_{t+1:t+T},\theta,x_t)= \sum_{k=1}^{N/T}\frac{1}{T}\sum_{l=1}^T ||\hat{y}_T-y_T||^2_2
\end{equation}

with $\hat{y}_T$ and $y_T$ are the predicted and ground truth values at time $t$, respectively.
\subsection{Trajectory classification}
The problem of learning the likelihood of an agent to follow a specific motion hypothesis can be formulated as a multilabel classification problem.
Given a series of observations $x^{(1)} \hdots x^{(T)}$ and a set of different trajectory classes $y$, we can train a classifier network to learn the likelihood of an agent following a certain hypothesis. %$\hat{y}$, given the true label $y$. 
The output of the network can be built by simply adding a fully connected layer (FC) at  the top of the LSTM network followed by an element-wise sigmoid activation function. Then, the \textit{log loss} can be used as the loss function:

\begin{equation}
    L(\hat{y},y,\theta,x_t)= \frac{1}{L}\sum_{l=1}^{L}-(y_l\cdot\log(\hat{y}_l)+(1-y_l)\cdot\log(1-\hat{y}_l))
\end{equation}

\subsection{Variational Autoencoder}
Variational autoencoder (VAE) belongs to the class generative models which can learn complex probabilistic models directly from data and perform inference. Consider the previous dataset %consisting of $N$ sample data points $\{x^{(i}\}_{i=1}^N$,
and that the observed variables \textbf{x} were generated from a underlying unobserved representation \textbf{z}. 

%Thus, the joint distribution  is defined as:
%\begin{equation}
%    p(\textbf{x},\textbf{z})= p(\textbf{x}|\textbf{z})p(\textbf{z})    
%\end{equation}

The goal of VAE is to learn probability distribution $p(\textbf{x})$ which can be obtained my marginalizing the joint distribution $p(\textbf{x},\textbf{z})=p(\textbf{x}|\textbf{z})p(\textbf{z})$ with respect to \textbf{z} resulting in:
\begin{equation}\label{eq:px}
    p(\textbf{x})=\int p(\textbf{x}|\textbf{z})p(\textbf{z})    
\end{equation}

There are two main problems with Equation \ref{eq:px} which make it extremely difficult to solve: the distribution of the latent space \textbf{z} is unknown, and the integral over the latent space when \textbf{z} is intractable.
%In order to solve Equation \ref{eq:px} there are two problems that need to be solved. Firstly, we need to define the latent variables $\textbf{z}$. In 
Generally, VAE's assume a prior over the latent space to be simple Gaussian distribution with zero mean and unit variance, $z\sim \mathcal{N}(0,I)$.
%VAE, define $\textbf{z}$ as $z\sim \mathcal{N}(0,I)$. 
Such assumption is only possible by employing a powerful function approximator, e.g. neural network, which can learn a non-linear map from the assumed Gaussian distribution to the observed \textbf{x}, resembling a \textit{decoder} structure in an autoencoder network. 

%Secondly, if \textbf{z} lies in a high dimensional space any approximation method to solve the integral of Eq. \ref{eq:px}, i.e. Monte Carlo sampling, would be unable to solve it due to its intractability. Thus, VAE's to apply another function approximator $Q(z|x)$ (\textit{encoder}) which is able to generate \textbf{z} values which are more likely to reconstruct \textbf{x}. One final step is still missing. In order to solve Eq. \ref{eq:px} we still need to sample values from $\textbf{z}$, of our encoder $Q(z|x)$ and decoder $P(x/z)$. Howeve
In addition, VAE parametrizes $p(\textbf{x}|\textbf{z})$ using another function approximator $Q(\textbf{z}|\textbf{x})$ (\textit{encoder}) of the posterior. Thus, by assuming that $Q$ generates \textbf{z} values more likely to reconstruct \textbf{x}, it resolves the intractable integral issue. Finally, the sampling operation necessary to solve  Eq. \ref{eq:px} is avoided by a reparametrizing $\textbf{z} = \boldsymbol{\mu} + \boldsymbol{\sigma}\odot \epsilon$.   The parameters $\phi$ of generative model $p(\textbf{x}|\textbf{z})$ and $\theta$ of the inference model $q(\textbf{z}|\textbf{x})$ can then be trained using standard backpropagation  by optimizing the following variational lower bound:
 
\begin{equation}
    \mathcal{L(\textbf{x},\theta,\phi)} - KL(q_{\phi}(\textbf{z}| \textbf{x})||p(\textbf{z})) + \mathbb{E}_{p(\epsilon)}[ \log{p_{\theta}(\textbf{x}|\textbf{z}=\boldsymbol{\mu} + \boldsymbol{\sigma}\odot \epsilon)}]
\end{equation}

with $KL(Q||P)$ as the Kullback-Leibler divergence between $Q$ and $P$, $\epsilon$ is a vector of Gaussian variables with independent marginal. 
%Typically, a prior over the latent random variable, $p(\textbf{z})$, is assumed to be a Gaussian distribution. However, if $\textbf{z}$ has high dimension Equation \ref{eq:px} becomes intractable. r, sampling is a discrete operation and does not allow to apply backpropagation to optimize the model in the parameter space. Kigma. et all. \cite{kingma2013auto}
% In simple terms, a VAE parametrizes $p(x|z)$ using a function approximator such as a neural network, introducing a highly non-linear mapping from \textbf{z} to \textbf{x} and resulting in a intractable inference of the posterior $p(\textbf{z}|\textbf{x})$.

\subsection{Baseline network}
The LSTM model proposed in \cite{Pfeiffer2017} is one of the first approaches incorporating three main sources of information influencing the agent navigation behavior: the query-agent state, the static-environment and surrounding agents. The first is the query-agent’s velocity $(v_x,v_y)$ represented in its local Cartesian coordinate frame. The second input is a 2D occupancy grid in a local neighbourhood $\pazocal{O}^i_{\textrm{static}}$, $n_s \times n_s $, of the agent and encoding information about the surrounding static obstacles. The latter consists of a vector array with the relative distance and velocity between the query-agent and the other agents.

% fusing information about the predicting agent, denoted as query-agent, environment and surrounding agents.
This approach can predict trajectories of pedestrians in crowded scenarios accurately. The proposed network architecture consists of three parallel input channels pre-processed in different ways. The information about the query-agent is fed directly to the network. In parallel, a compressed representation of the static environment is generated by feeding the static grid into an encoder network, previously pre-trained using an auto-encoder scheme. Finally, the information about the surrounding agents is fed through a fully connected layer (FCL). Then, an LSTM layer is stacked in front of each input channel learning the time-dependencies. The output of each LSTM is concatenated creating a latent representation of the three input channels. Finally, another LSTM layer is stacked, learning the time-dependencies of the latent space. The output of the model is the predicted velocities for the query-agent for a prediction horizon $T$ resulting in the following loss function:

%where the velocity of each agent at each time step is used to update the internal representation of the model. 
%Our baseline approach uses a $\textit{L}$2-norm loss function only learning the average behavior of the pedestrians.

\begin{equation}
    L(\theta,v^i)=\frac{1}{T}\sum_{l=1}^T||\hat{v}^i_l-v^i_l||+\lambda\cdot \alpha(\theta)
\end{equation}
with $v^i$ represents the ground truth velocity for the i-th agent, $\hat{v}^i$ the model predicted velocities, $\alpha(\theta)$ and $\lambda$ the regularization terms and the regularization factor, respectively. For more details about the network architecture, we refer the reader to \cite{Pfeiffer2017}.
%Our baseline model incorporates three main sources of information influencing the agent navigation behavior: query-agent states, the environment and social context \cite{Pfeiffer2017}. The first is the query-agent’s velocity $(v_x,v_y)$ represented in its local Cartesian coordinate frame. The second input is a 2D occupancy grid in local neighborhood $\pazocal{O}^i_{\textrm{static}}$, $n_s \times n_s $, of the agent and encoding information about the agent surrounding environment. The last consists of a vector array with the relative distant and velocity between the query-agent and the others.

%We employ a Recursive Neural Network (RNN) model
